Skill Disentanglement for Imitation Learning from Suboptimal Demonstrations

Imitation learning has achieved great success in many sequential decision-making tasks, in which a neural agent is learned by imitating collected human demonstrations. However, existing algorithms typically require a large number of high-quality demonstrations that are difficult and expensive to collect. Usually, a trade-off needs to be made between demonstration quality and quantity in practice. Targeting this problem, in this work we consider the imitation of sub-optimal demonstrations, with both a small clean demonstration set and a large noisy set. Some pioneering works have been proposed, but they suffer from many limitations, e.g., assuming a demonstration to be of the same optimality throughout time steps and failing to provide any interpretation w.r.t knowledge learned from the noisy set. Addressing these problems, we propose {\method} by evaluating and imitating at the sub-demonstration level, encoding action primitives of varying quality into different skills. Concretely, {\method} consists of a high-level controller to discover skills and a skill-conditioned module to capture action-taking policies, and is trained following a two-phase pipeline by first discovering skills with all demonstrations and then adapting the controller to only the clean set. A mutual-information-based regularization and a dynamic sub-demonstration optimality estimator are designed to promote disentanglement in the skill space. Extensive experiments are conducted over two gym environments and a real-world healthcare dataset to demonstrate the superiority of {\method} in learning from sub-optimal demonstrations and its improved interpretability by examining learned skills.

==> secs/problem_setting.tex <==
\section{Preliminary}

\subsection{Problem Setting}

\suhang{it is a little bit strange that we start with the technique MDP. Can we start with the data and motivation examples?}In this work, we consider the standard fully Markov Decision Process (MDP) setting~\cite{sutton1998reinforcement}, $\mathcal{M}=\{\mathcal{S}, \mathcal{A}, T, R, \gamma, \rho_0 \}$. $\mathcal{S}, \mathcal{A}$ are the state space and action space respectively, $T: \mathcal{S} \times \mathcal{A} \times \mathcal{S} \rightarrow [0,1]$ is the MDP's transition probability, $R: \mathcal{S}\times \mathcal{A}\rightarrow \sR$ is the reward function, $\gamma \in [0,1)$ is the discount factor for future reward and $\rho_0$ is the distribution of initial states. A policy $\pi: \mathcal{S} \times \mathcal{A} \rightarrow [0,1]$ maps the observed state to a probability distribution over actions. Following the standard IL setting, the reward function $R$ is not available. Instead, we aim to learn a policy $\pi_\theta$ from the collected demonstration set. Each demonstration is a trajectory, a sequence of state-action pairs (transitions) $\tau = (\vs_0, \va_0, \vs_1, \va_1, ... )$, with $\vs_t$ and $\va_t$ being the state and action at time step $t$. 

Most existing imitation learning works assume that these demonstrations are all optimal, collected from domain experts. However, it is usually challenging to collect a sufficiently large expert demonstration set. Concretely, we have a small clean demonstration set $\mathcal{D}^{clean} = \{\tau_i\}_{i=1}^{n_{e}}$ which is drawn from the expert optimal policy $\pi_e$\suhang{can you give some example of the expert optimal policy in real-world}, and a larger noisy demonstration set $\mathcal{D}^{noisy} = \{\tau_i\}_{i=1}^{n_{o}}$ generated from some other offline \suhang{what does the offline policy means here?} behavior policies\suhang{can you give an example of the offline behavior policy}. Note that these offline policies could be much worse than the expert policy $\pi_e$. In this task, we want to learn a policy agent $\pi_{\theta}$ by extracting useful information from both optimal demonstrations $\mathcal{D}^{clean}$ and noisy demonstrations $\mathcal{D}^{noisy}$. \suhang{Tianxiang, can you come up with one example we can use throughout the paper to explain these notations, including the trajectory, state, optimal policy, offline policy, noisy trajectory, .... An example would be easier to help readers understand and convince the readers}

We assume that these demonstrations are generated from semantically meaningful skills\suhang{again, can you be more concrete, preferably with an example}, with each skill encoding a specific action primitive, a sub-policy. Demonstrations in $\mathcal{D}^{noisy}$ can be split into multiple segments, and useful information can be extracted from segments that are generated from high-quality skills.

\subsection{Mutual Information} 
Mutual information (MI) measures the mutual dependence between two variables from the information theory perspective. For random variables $X$ and $Y$, their mutual information score can be computed as:
%\begin{equation}\label{eq:MI}
%    I(X, Y) = \int_{\sX \times \sY} log\frac{dP_{XY}}{dP_X \otimes P_Y} dP_{XY},
%\end{equation}
\begin{equation}\label{eq:MI}
    I(X, Y) = \int_{\sX}\int_{\sY} P_{XY}(\rx,\ry) log\frac{P_{XY}(\rx,\ry)}{P_X(\rx) \otimes P_Y(\ry)} d\rx d\ry,
\end{equation}
in which $P_{XY}$ is the joint distribution probability, and $P_X = \int_\sY P_{XY}d\ry$ and $P_Y = \int_\sX P_{XY}d\rx$ are the marginals. Methods based on MI have a long history in unsupervised learning, following the infomax principle~\cite{bell1995information,linsker1988application} and leveraging known structures in the input. For example, ~\cite{bell1995information} maximizes MI between the input and output, ~\cite{hu2017learning} optimizes MI among representations obtained from data augmentations and other transformations to avoid degenerate solutions, and ~\cite{hjelm2018learning} maximizes MI between representation obtained from global and local scales. 

Computation of mutual information in Eq.~\ref{eq:MI} is usually intractable for continuous variables in the real world due to the integral. MINE~\cite{belghazi2018mutual} proposes a neural estimator that can be learned to provide its lower bound, derived from the duality theory. Following MINE, a Jensen-Shannon MI estimator is proposed in ~\cite{hjelm2018learning} which offers better stability in optimization:
\begin{equation}
\begin{aligned}
   \widehat{I}^\text{(JSD)}(X, Y) := &\max_{\omega} \E_{P_{XY}}[-\text{sp}(-T_{\omega}(\rx, \ry))] \\
    &- \E_{P_X \otimes P_Y}[\text{sp}(T_{\omega}(\rx, \ry))],
    \label{eq:MI_JS}
\end{aligned}
\end{equation}
in which $\text{sp}(\rx) = \log(1 + e^\rx)$ is the softplus function, and $T_{\omega}: \sX \times \sY \rightarrow \R$ is a discriminator function modeled by a neural network with parameters $\omega$.

%In this work, we target to discover latent skills or action primitives behind collected demonstrations, hence we propose to maximize MI between discovered skill variables and state-action pairs. Details will be introduced in the next section.


